T-Crowd: Effective Crowdsourcing for Tabular Data

Crowdsourcing employs human workers to solve computer-hard problems, such as data cleaning, entity resolution, and sentiment analysis. When crowdsourcing tabular data, e.g., the attribute values of an entity set, a worker's answers on the different attributes (e.g., the nationality and age of a celebrity star) are often treated independently. This assumption is not always true and can lead to suboptimal crowdsourcing performance. In this paper, we present the T-Crowd system, which takes into consideration the intricate relationships among tasks, in order to converge faster to their true values. Particularly, T-Crowd integrates each worker's answers on different attributes to effectively learn his/her trustworthiness and the true data values. The attribute relationship information is also used to guide task allocation to workers. Finally, T-Crowd seamlessly supports categorical and continuous attributes, which are the two main datatypes found in typical databases. Our extensive experiments on real and synthetic datasets show that T-Crowd outperforms state-of-the-art methods in terms of truth inference and reducing the cost of crowdsourcing.

==> methodology.tex <==
%!TEX root = main.tex

\section{methodology}\label{sec:methodology}


\subsection{Problem Formulation}
We start by defining our framework for collecting structured data. 


\begin{definition}

There is an empty or partially-filled table $X$. The row of table corresponds to a object or fact and the column is a property or attribute which is used to describe the object or fact. 

\end{definition}

Our goal is to fill in the whole table with high quality, low cost and latency.


\begin{example}

Table 1 is about country information. Each row is a country and each column is a property of country. We has known the values in several cells while missing the other values. 
\end{example}

\begin{table*}[]
\centering
\caption{Country Infomation}
\label{countryInfo}
\begin{tabular}{|c|c|c|c|c|l|}
\hline
              & Population    & Area      & Founded Time & Capital & Currency \\ \hline
China         & 1,376,049,000 &           &                              & Beijing &       \\ \hline
United States &   322,014,853            & 9,857,306 &  1776                            &         &       \\ \hline
India         &               &           &                   &         &          \\ \hline
\end{tabular}
\end{table*}

\begin{definition}

A cell is the smallest part in the table $X$ and cell $X_{ij}$ is decided by the object $i$ and attribute $j$.
An annotation $A_{ij}^{u}$ is a piece of information provided by a worker about a given cell $X_{ij}$. A truth $T_{ij}$ is the most trustworthy piece of information for a cell. 

\end{definition}

\begin{definition}
The attributes in the table can be divided into two types: categorical or continuous. Categorical attribute is that the truth is from a fixed set of possible values, and each values have no magnitude. Continuous attribute is that truth is an integer or real value and has magnitude. The domain of continuous attribute is $[-\infty,+\infty]$ and Categorical attribute is a fixed label set $L=\{L_1,L_2,...,L_V\}$.
\end{definition}

\begin{example}

In Table 1, Population, Area and Founded Time are the continuous attributes while Capital and Currency are Categorical attributes.   
\end{example}

Now we have the set of annotations $A_{ij}^{u}$ that can be taken as input. We want to obtain the ground truth $T_{ij}$ in the whole table as output.

\subsection{Worker Modeling}



\subsection{Task Modeling}
